Neural Rendering based Urban Scene Reconstruction for Autonomous Driving

Dense 3D reconstruction has many applications in automated driving including automated annotation validation, multimodal data augmentation, providing ground truth annotations for systems lacking LiDAR, as well as enhancing auto-labeling accuracy. LiDAR provides highly accurate but sparse depth, whereas camera images enable estimation of dense depth but noisy particularly at long ranges. In this paper, we harness the strengths of both sensors and propose a multimodal 3D scene reconstruction using a framework combining neural implicit surfaces and radiance fields. In particular, our method estimates dense and accurate 3D structures and creates an implicit map representation based on signed distance fields, which can be further rendered into RGB images, and depth maps. A mesh can be extracted from the learned signed distance field and culled based on occlusion. Dynamic objects are efficiently filtered on the fly during sampling using 3D object detection models. We demonstrate qualitative and quantitative results on challenging automotive scenes.

==> archived/algorithm.tex <==
\section{PROPOSED ALGORITHM AND RESULTS} \label{sec:algo}
% \LYc{@Michal: could you review this section please?}

In this section, we describe the system perspective context (Section~\ref{subsec:system_perspective}), then the two proposed algorithms, specifically the image processing baseline (Section~\ref{subsec:first_solution}) and the CNN baseline (Section~\ref{subsec:cnn}).

\subsection{System Perspective} \label{subsec:system_perspective}
% \LYc{@Michal: could you review this section please?}

% \SY{this section positions where sun glare fits in overall system. We discuss MTL to do joint CNN model for sun glare and discuss fusion too. Its better this way than saying future work.}
% \MUc{To be honest, I think that MTL for both sun glare and soiling is a bullshit. Its unnecessary over-complication of something which could be neatly solved via semantic segmentation enhanced by additional classes for sun glare and soiling. The interesting open problem is then how to tackle the problems with unreliable annotations.}
% \SY{Soiling and sun glare could be added as separate classes in segmentation but the reason we don't is to decouple it and have full control for dataset design for soiling and sun glare. this is why we do it this in icam3. @michal, is tat ok? we dont have additional classes dataset anyways?}
% \MUc{Well, from the project point of view, there is some logic behind this. However, from scientific point of view, this means we are doing some pseudo hacks. If we would approach the problem from the ground up, we could have the same degree of control without decoupling. Another benefit of having this handled by semantic segmentation is increase in processing speed.}

Deploying a single network dedicated only for one task is always expensive on any embedded platform. Recent trends of Multi Task Learning (MTL) for vision based tasks can be leveraged in this case. As the sun glare detection task is quite different than other perception tasks such as semantic segmentation, object detection etc., so we plan to use a pre-trained shared encoder and task specific decoders to train the sun glare detection task as a separate decoder as shown in Figure~\ref{fig:mtl_sunglare}.

As a step towards making sun glare detection more robust, the output from classical algorithm and predictions from CNN can be fused  using uncertainty map. This will lead us to achieve sun glare tracking.
% \LYc{@Senthil: Can you answer Michal's comment please?}
% \AD{@Lucie: It was a mistake from my side, I changed it to sun-glare tracking}
By merging the sun glare detection as a part of other vision based tasks through MTL, we can reduce the computation complexity at least by half \cite{sistu2019neurall}. This way the pre-trained shared encoder can be used as an efficient feature extractor that has good understanding of the automotive scenes during the training of other tasks. Our baseline of semantic segmentation and object detection network details are described in \cite{sistu2019real,chennupati2019multinet++}. Besides, end-to-end joint training of all tasks can be done to see the impact on KPI of other decoder outputs due to the addition of the sun glare detection. 
% However,  major challenges in doing this involve a creation of simultaneous annotation for all tasks and design of a proper loss function.

% \begin{figure}[!h]
\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{images/algorithm/fusion.png}
    \caption{Fusion of image processing and CNN results using uncertainty map
    }
    \label{fig:fusion}
\end{figure}


Based on the problem explained in the previous section, we are proposing a new method for sun glare detection (direct or indirect sun glare) by combining information given by image processing filters and multi-camera tracking. This can be used to either enhance processing in this region, change tracking criteria to limit the system functionality, or to simply inform the system about a threat of a potential performance degradation. An example of this would be camera based lane sensing on a straight wet road with the vehicle travelling towards the sun which is low in the sky. In this case, detection accuracy and range would be severely impacted and hinder the lane assist functionality severely.

% \AD{Need to check with LY about the meaning of these two sentences. Maybe it needs explanation in a bit more details.} 
% \say{This use case good induce a negative impact on the detection performance ahead of the vehicle. Detection of such a scenario in an autonomous system could enforce a restriction on the maximal speed or prevent overtaking maneuvers because of the reduced detection range.}
% \LYc{Please check with Senthil as he wrote that paragraph :)}


% Our proposed method automatically detects and tracks sun glare using information given by different modules \AD{@Lucie: can you please look into this sentence? I think it needs restructuring. it is better to be very specific about the \say{different modules}} \LYc{Please check with Senthil as he wrote that paragraph :)} already in the vehicle.



\subsection{First Solution: Image Processing Algorithm} \label{subsec:first_solution} %\LY{LY}
% \LYc{@Michal: could you review this section please?}

% \begin{figure}[!h]


An image processing algorithm is used to detect sun glare using different processing blocks, such as color conversion, adaptive thresholding, geometric filters and blob detection. By getting information from image processing, we can find a redundancy between regions detected as saturated using image processing and CNN output.
This image processing algorithm is different than the annotation algorithms as thresholds and morphological operations applied are different. To avoid having the same issue as the one encountered in the automatic annotation algorithm, such as white objects detected as sun glare, thresholds, morphological operations and blob detection blocks are used using sharper values.

\begin{figure}[tb]
    \centering
    \includegraphics[width=\columnwidth]{images/algorithm/algImgProcessing.png}
    \caption{Image processing algorithm scheme}
    \label{fig:imgProcessing}
\end{figure}

First, the image is converted into the YUV color space before applying a threshold in order to get only pixels that are potentially over-exposed (pixel value of $255$). 
To remove noise, a closing operation has been applied followed by an erosion operation which removes small objects so that only substantive objects remain. The blob detection step starts by finding the contours using the method that stores all the contour points and the mode to retrieve only the outer contours. Finally, polygons are created using the convex hull method. The size of the polygon is checked as we do not want to detect sun glare regions that are smaller than a specified threshold. This size differentiation removes some of the false detections. The Figure~\ref{fig:imgProcessing} shows the steps of this image processing algorithm.
% \LYc{Why is the image so far away from the text?}
% \MUc{Don't worry about that, we will polish the placement once the text is finalized as till that time it will be moving anyway.}
% \MUc{I think we should add more details here. After reading, I am not sure if I could re-implement this.} \LYc{I did not add much more details because it is a very simple algorithm so I don't know if it worth to detail it :/ What do you think?}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.85\linewidth]{images/cnn/MTLSunglare.png}
    \vspace{1mm}
    \caption{Illustration of how sun glare detection CNN model will be part of a pre-trained Multi-Task Learning model}
    \label{fig:mtl_sunglare}
\end{figure*}

\noindent The algorithm has been tested on $300$ images from the test set and KPIs (Key Performance Indicators) have been determined as follows:
% \MUc{Why is TN ommited? Also, do we really make decisions based on all these, or we can simplify by using only e.g. F1-score?} \LYc{Do you suggest I add precision (0.85) and recall (0.96) instead of TP, FP and FN? I can calculate TN as well but as it is sun glare detection, I thought that it was not really relevant to add TN (average = 99.4, median = 99.5), but if you think it is, then I will :)}
\begin{itemize}[nosep]
    \item[--] True Positive (TP): proportion of pixels detected and annotated as ``sun glare''.
    \item[--] False Positive (FP): proportion of pixels detected as “sun glare” but annotated as “no sun glare”.
    \item[--] False Negative (FN): proportion of pixels detected as “no sun glare” but annotated as “sun glare”.
    \item[--] True Negative (TN): proportion of pixels annotated and detected as "no sun glare" 
    \\
    % \item[--] \(Precision = \frac{TP}{TP + FP}\)
    % \item[--] \(Recall = \frac{TP}{TP + FN}\)
    %\item[--] Precision: ratio of pixels predicted as "sun glare" and annotated as sun glare
    %\item[--] Recall: ratio of correctly predicted positive observations to the all observations in actual class
\end{itemize}


From the the KPIs detailed in the previous list, precision (\(Precision = \frac{TP}{TP + FP}\)) and recall \(Recall = \frac{TP}{TP + FN}\) metrics have been calculated.
\begin{itemize}[nosep]
    \item [--] \(Precision = 85\% \)
    \item [--] \(Recall = 96\% \)
\end{itemize}


% \begin{table}[tb]
%     \vspace{5mm}
%     \caption{TODO \SY{do one table for both CNN and IP}}
%     % \begin{adjustbox}{width=0.9\linewidth}
%     \label{tab:precisionRecall}
%     \begin{tabular}{|c|c|}
%         \hline
%         Precision & 85\% \\
%         Recall & 96 \% \\
%         \hline
%     \end{tabular}
%     % }
%     % \end{adjustbox}
% \end{table}


\subsection{Second solution: CNN} \label{subsec:cnn} 
% \LY{MU + AD + PK}
% \LYc{@Michal: could you finish this section please?}

% We exploit the annotations provided by the image processing algorithm described in Section~\ref{subsec:first_solution} and use it as a ground truth for end-to-end fully supervised training of the fully convolutional neural network. \LY{We used the images coming from annotation for GT, not the output from IP alg} 

We make use of the WoodScape sun glare dataset ground truth for training a fully convolutional neural network. 
In Figure~\ref{fig:MaskSegNet}, we depict the CNN's architecture, the building blocks are denoted as follows: convolution blocks (blue in the Figure~\ref{fig:MaskSegNet}) encode the kernel size, stride, number of output channels, following type normalization (if any) and an activation layer. So, ``c7s1-32-IN-R'' reads as a 2D convolution layer with kernel size $7$ pixels, stride $1$ pixel, $32$ output channels, followed by instance normalization layer and ReLU activation layer. ``S'' in the last convolution block stands for the Sigmoid activation layer; residual block (purple in Figure~\ref{fig:MaskSegNet}) consists of a 2D reflection padding layer, followed by a 2D convolution layer with kernel size $3$, the same number of input channels as the output channels ($64$), followed by the batch normalization layer and ReLU activation; finally, upscaling block (yellow in Figure~\ref{fig:MaskSegNet}) is a nearest-neighbor upsampling layer by a factor of $2$.




We train our network via Adam optimizer~\cite{kingma2014adam} with learning rate set to $1\times10^{-4}$, $\beta_1 = 0.9$, $\beta_2 = 0.999$, and $\epsilon = 1\times10^{-8}$, we let the network train for $200$ epochs. As the loss function evaluating the necessary gradient changes, we use the cross entropy loss. To better utilize the small number of training samples, we use the simple data augmentation consisting of random cropping with $12\%$ in both width and height, random horizontal and vertical flipping, and random rotation by $180^\degree$. The probability of all augmentations is set to $0.5$, except of the random cropping, which happens always. Since the annotations are not $100\%$ precise and due to lack of data, we let the network to be trained for full $200$ epochs, without formulation of any reasonable stopping criterion. 

\begin{table}[tb]
    \vspace{5mm}
    \caption{True Positive (TP), False Positive (FP), True Negative (TN) and False Negative (FN)}
    \begin{adjustbox}{width=0.9\linewidth}
    \label{tab:TPTNFPFN}
    \begin{tabular}{|c|c||c|c|}
        \hline
        Average TP & 96.23\% & Average FP & 16.41\% \\
        Median TP & 97.49\% & Median FP & 18.2\% \\  
        \hline
        Average FN & 3.8\% & Average TN & 99.4\%\\ 
        Median FN & 2.5\% & Median TN & 99.5\%\\
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

% \MUc{TODO: cross entropy loss, evaluation on test data --- mean Intersection over Union and its disadvantages}
For evaluation on the test set, we opted for the commonly used mean Intersection over Union (mIoU), also known as the Jaccard score. However, we noticed there are several problems in our specific task which concerns usage of imprecise ground truth labels. Theoretically, there are $4$ distinct cases that might occur in sun glare semantic segmentation IoU evaluation. However, one is highly unlikely as it covers the case when whole image would belong to the sun glare class. Therefore, we will limit ourselves to only three common cases. The first case is when both classes are represented in both ground truth label and the prediction. The second case is formed by an image which is not affected by sun glare and correctly recognized as such (i.e. both ground truth and prediction are represented only by ``clean'' label). The last, third, case is described by a situation when sun glare is detected in a ``clean'' image. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.33\linewidth]{images/cnn/MaskSegNet}
    \vspace{1mm}
    \caption{Proposed sun glare CNN architecture. Description of individual components is in the text.}
    \label{fig:MaskSegNet}
\end{figure}



\begin{table}[tb]
    \vspace{5mm}
    \caption{Results from the CNN experiment. Each case is detailed in the text. Class 0: Background | Class 1: Sun glare}
    \begin{adjustbox}{width=0.9\linewidth}
    % \centering
    
    \label{tab:CNNresults}
    \begin{tabular}{|c|c|c|c|c|c|c|}
        \hline
        CASE 1 & IOU & mean & std & median & min & max \\ 
        Class 0 & 99.01 & 98.46 & 1.04 & 98.94 & 94.91 & 99.73 \\  
        Class 1 & 51.28 & 51.49 & 13.68 & 51.19 & 8.06 & 77.76 \\ 
        \hline
        \hline
        CASE 2 & IOU & mean & std & median & min & max \\ 
        Class 0 & 100 & 100 & 0 & 100 & 100 & 100 \\  
        Class 1 & 100 & 100 & 0 & 100 & 100 & 100 \\  
        \hline
        \hline
        CASE 3 & IOU & mean & std & median & min & max \\ 
        Class 0 & 0 & 0 & 0 & 0 & 0 & 0 \\  
        Class 1 & 0 & 0 & 0 & 0 & 0 & 0 \\  
        \hline
    \end{tabular}
    \end{adjustbox}
\end{table}

The problem is that in the last case, the mIoU does not reflect how bad the prediction was. 
In our experiments, we frequently spot incorrect classification of sun glare in just a few pixels, however in terms of the mIoU, this leads to radical drop towards $0.5$. Another problem is the imprecise annotation, which affects the first case as well--- since the labels are imprecise, mIoU going to $1.0$ is actually not good.

% \MUc{TODO: problematic is the last case which is sort of a corner case. First one is problematic as well, due to imprecise ground truth labels.}
% \MUc{We consider our proposed solution rather a first baseline. We want to investigate the possibilities of weak supervision to tackle these issues.}

We would like to emphasize that we are aware of the limits of the proposed approach and consider it as a baseline solution. We want to investigate the possibilities of a weak supervision, providing a more principled way of dealing with the aforementioned issues. 

% \MU{
% \cite{deeplab-TPAMI-Chen-2018, Zhu-ICCV-2017, chen2018encoder, he2016deep, Shelhamer-2017}
% }

\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{images/results.png}
    \vspace{0.1mm}
    \caption{The visual comparison of several testing examples. Left to right: original RGB image, ground truth annotation, CNN prediction.}
    \label{fig:cnn_results}
\end{figure}

\subsection{Discussion} \label{subsec:discussion} 

The goal of this work is to emphasize the importance of the sun glare detection which is relatively less explored in automated driving. To enable further research, we created a dataset comprising of diverse and challenging scenarios. We implemented two basic prototypes using traditional image processing and deep learning. The false positive rate of $16\%$ in the image processing approach demonstrates that the problem is not easily solvable using a simple classical approach. To our surprise, the semantic segmentation model achieves only a moderate IoU of $51$ for sun glare regions. We outlined the problems with the mIoU metric, which explain this ``low performance''. However, it also  demonstrates that the sun glare detection is a challenging problem and needs a larger design effort. We see it also as an opportunity for further investigation by the community. 
%It also shows that our dataset is not already saturated with simple approaches and there is an opportunity in the community for further research. In particular, sun glare regions do not have sharp boundaries and there is typically some errors in these regions. 
% MU: we cannot say this, if we say there is a problem of inprecise annotations, we cannot leverage it at the same time, saying that the problem is not resolved by simple approaches :) 



==> archived/conclusions.tex <==
\section{Conclusion} \label{sec:conclu}
Sun glare detection is an important problem for higher levels of automated driving. But this topic is not explored in detail in the community as there is no public dataset available. Thus we created a new dataset and will release it as a part of the WoodScape project \cite{yogamani2019woodscape}. We developed two prototypes using CNN and classical image processing approach and we intend it to be baselines for the dataset. In future work, we plan to perform a fusion of both approaches and also integrate the CNN model into a multi-task network.

% TODO

% Sun glare is an important topic for human and autonomous driving scenarios

% Limitation of the annotation technique

% Image processing and CNN give promising results
% Image processing gives good TP but bad FP
% CNN is failing in transition areas


% \SY{suggest write only one or two sentences for future work, we will either not do it or its not good to give out the ideas :)}

% \AD{Done}

% \textbf{Future Work:}

% A more meaningful annotation technique needs to be defined due to various reasons. Sun-glare is not well defined, hence quite hard to annotate. Besides, a new KPI should be defined that represents the problem well. It is not very clear what is the correct boundary of a sun-glare as there is a smooth transition between strong sun-glare to no sun-glare. Due to absence of sharp boundary, annotated mask may not match with the predicted one, so there will always be error amounting in mIoU.






==> archived/dataset.tex <==
\section{DATASET DESIGN } \label{sec:Dataset}
% \LYc{@Arindam: could you review this section please?}
% \AD{Done}

This section explains how the sun glare dataset has been created. Section~\ref{sec:Dataset Design} provides the requirements of the dataset. Section~\ref{sec:Dataset Details} explains the methods used to do annotation. Finally, Section~\ref{sec:WoodScape} describes the WoodScape~\cite{yogamani2019woodscape} dataset, in which the sun glare dataset will be made available to the public in the next few months.


\subsection{Dataset Design} \label{sec:Dataset Design}
% \LYc{@Arindam: could you review this section please?}
% \AD{Done}

A dataset that contains images with sun glare effects has been created as to the best of our knowledge there are no public datasets available to address the presented problem. 
Fisheye cameras are widely used in the automotive industry because they offer a wide field of view (FoV). Four cameras are installed on a moving vehicle capturing the full surround view of the vehicle (one front view, two side-mirror views and one rear view). The dataset is composed by images recorded in two different countries.
The typical scenarios we are interested in are when the sun glare is present on an image (in the sky and/or on the road) from one of the cameras. 
The following list gathers different scenarios of sun glare and details the dataset content:
\begin{itemize}[nosep]
    \item Sun glare due to the reflection of the Sun on the ground plane (whatever the surface: road, water, snow, etc.).
    \item Sun glare regions that are due to the reflection of the Sun on vertical objects with specular surface/material (e.g.: cars, trucks, signs, etc.).
    \item Sun glare due to direct Sun.
    \item Sun glare regions on the car body of the ego vehicle due to the Sun.
    \item Images without Sun glare.
\end{itemize}
  
\subsection{Dataset Details} \label{sec:Dataset Details}
% \LYc{@Arindam: could you review this section please?}
% \AD{Done}

% \begin{figure}[!t]
\begin{figure}[tb]
    \centering
    
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=0.45\columnwidth]{images/dataset_img/dataset_01.png}
    \includegraphics[width=0.45\columnwidth]{images/dataset_img/dataset_mask_01.png}
    \caption{Left: Image annotated with sun glare regions. Right: Corresponding mask annotation}
    \end{subfigure}
    
    \vspace{4mm}
    
    \begin{subfigure}{0.5\textwidth}
    \centering
    \includegraphics[width=0.45\columnwidth]{images/dataset_img/dataset_02.png}
    \includegraphics[width=0.45\columnwidth]{images/dataset_img/dataset_mask_02.png}
    \caption{Left: Image annotated with sun glare regions. Right: Corresponding mask annotation}
    \end{subfigure}
    
    \vspace{4mm}
    
    \caption{Examples of images annotated}
    \label{fig:datasetEx}
\end{figure}

It is very difficult to annotate a sun glare as there are no definite boundaries around them. A sun glare, as defined in the earlier section, is a part of the image, where the pixels are over-exposed. This is why it has been chosen to annotate the dataset using automatic annotation followed by a manual check. 
Some image processing techniques, for example thresholding and morphological operations are used to detect regions where the sun glare effect is found more than likely. Unfortunately, the polygons created using this technique do not differentiate the sun glare effect with other very bright/white objects in the image. This is why a manual check was added in the annotation process. Each image has been visually checked by an annotator and decision such as discarded/validated was made.
The created dataset has been split into two parts~\cite{Uricar-2019b}: a training set which contains around $1,115$ images ($580$ images with sun glare and $535$ images without sun glare), and a test set of around $294$ images ($184$ images with sun glare and $110$ without sun glare regions). Uncertainty maps with probability per pixel for each images are provided as well. The Figure~\ref{fig:datasetEx} is showing example of the annotation.


\subsection{WoodScape} \label{sec:WoodScape}

WoodScape is a comprehensive multi-task multi-camera fisheye dataset for automated driving. Figure~\ref{fig:woodscape} illustrates various tasks planned to be part of the release. It comprises of classical vision tasks such as object detection and semantic segmentation, and geometric tasks like depth estimation and motion estimation. We would like to augment this dataset to include sun glare task as well. Sun glare dataset images are completely separate from other datasets. This is the reason we explore it as a separate task rather than augmenting it with segmentation where sun glare region is an additional class. This way the dataset design for sun glare can be flexible and extensive without coupling with other tasks. Annotation formats and folder structures for sun glare task will be consistent with other tasks. 


\begin{figure*}[tbh]
    \centering
    \includegraphics[width=2\columnwidth]{images/woodscape_tasksOverview.PNG}
    \vspace{1mm}
    \caption{Illustration of the main tasks in our WoodScape dataset \cite{yogamani2019woodscape}}
    \label{fig:woodscape}
\end{figure*}




==> include/related.tex <==
\section{RELATED WORK} \label{sec:related}

% \noindent \textbf{Optical Flow Estimation:} Traditional solutions have been studied and adapted for decades~\cite{horn1981determining, brox2004high}. In order to be robust against more challenging open world problems including lack of features, motions in different scales, and occlusions, recent learning-based methods outperform traditional ones. Dosovitskiy et al.~\cite{dosovitskiy2015flownet} propose FlowNetS and FlowNetC, which is a pioneer work in showing the feasibility of directly estimating optical flow given images. Sun et al.~\cite{sun2018pwc} design PWC-Net, a much more efficient solution based on pyramidal processing, warping and the use of a cost volume. RAFT~\cite{teed2020raft}, proposed by Teed and Deng, demonstrates notable improvement by building multi-scale 4D correlation volumes for all pairs of pixels and iteratively updating flow estimates through refinement module based on gated recurrent units (GRU). All these methods are fully supervised and trained using imagery from a standard pinhole camera. The training data are also collected during the day with sufficient brightness. None of them pays attention to the performance of optical flow in more challenging AV applications such as strong lens distortion and driving at night, which leads to errors and even catastrophic failures. 
% \vspace{3pt}


% \noindent \textbf{Strong Lens Distortion:} There is very limited work on perception tasks for strongly distorted images such as fisheye images. Popular approaches include rectifying the radial distortion before passing images into any regular perception pipeline. However, this will inevitably bring reduced field-of-view and resampling distortion artifacts especially at the image borders~\cite{kumar2021svdistnet}. Spatially variant distortion that makes closer objects appear larger also poses scaling problems and complexity to geometric perception tasks. Additionally, Rashed et al.~\cite{rashed2021generalized} show that the common use of bounding boxes for object detection no longer fit well for rectangular objects in distorted images. More sophisticated representations for detected objects, such as a curved bounding box exploiting the known radial distortion, are explored in~\cite{rashed2020fisheyeyolo}. Although there is some literature using distorted images without rectification on other perception tasks, such as depth estimation~\cite{kumar2018near, kumar2020fisheyedistancenet}, soiling~\cite{uricar2019desoiling}, visual odometry~\cite{liu2017direct} and multi-task models~\cite{leang2020dynamic, kumar2021omnidet}, there is no previous work estimating optical flow due to the difficulty in labeling ground truth. WoodScape~\cite{yogamani2019woodscape}, KITTI 360~\cite{liao2022kitti} and Oxford RobotCar~\cite{maddern20171} are some well-known autonomous driving datasets containing strongly distorted images such as fisheye images, but none of them has optical flow ground truth. In this paper, we take advantage of the synthetic fisheye dataset published recently, SynWoodScape~\cite{sekkat2022synwoodscape}, which is the first dataset providing optical flow for both foreground and background motions by computing it analytically using other data modalities extracted from the simulator. We train our network using synthetic data from SynWoodScape and evaluate it on real-world fisheye data from WoodScape.
% \vspace{3pt}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width = 2\columnwidth]{images/results/fisheye_qual.jpg}
%     \vspace*{1mm}
%     \caption{Optical flow estimation (color coded) on real-world automotive data from WoodScape~\cite{yogamani2019woodscape}. Input frames are from the fisheye cameras of front view, right-side view, and left-side view respectively. }
%     \label{fig:fisheye}
% \end{figure*}

% \noindent \textbf{Low-Light Scenes:} Similar to optical flow estimation on strongly distorted images, there is some work handling low light in a few perception tasks~\cite{rashed2019fusemodnet, alismail2016direct, ge2009real} but none of them has proposed an optical flow estimation algorithm that is robust against low-light scenes. Very related to ours, Zheng et al.~\cite{zheng2020optical} propose a method to synthesize low-light optical flow data by simulating the noise model on dark raw images, which is then used to finetune an off-the-shelf network. However, their method is not able to synthesize more realistic characteristics of real-world low-light scenes one would observe in AV applications, such as the motion blur and local illumination changes brought by multiple light sources. Their improvement is also very limited due to the off-the-shelf network is not designed nor trained to learn nighttime-robust representations. In addition, a variety of techniques have been developed for low-light image enhancement~\cite{chen2018learning, lv2018mbllen} and image-to-image translation~\cite{liu2017unsupervised, huang2018multimodal}. The former can preprocess inputs to a flow estimation network during inference by brightening up a given low-light image, whereas the latter can translate a daytime image into its nighttime counterpart so as to complement the lack of optical flow datasets in low light~\cite{rashed2019fusemodnet}. But neither approach facilitates the network training in that the processed data bring in extra complexities such as additional artificial noise, overexposure, or inconsistent image translation across frames. Finally, semi-supervised learning is a common approach to tackling the lack of optical flow data in particular scenarios, where a set of predefined transformations are applied to the original labeled data and the output of the perturbed data are enforced to agree with the outputs of the original data~\cite{laine2016temporal}. For example, Jeong et al.~\cite{jeong2022imposing} use a semi-supervised setup to impose translation and rotation consistency equivariance for optical flow estimation. Yan et al.~\cite{yan2020optical} synthesize foggy images from clean and labelled images in order to avoid flow estimation errors caused in dense foggy scenes. Similar to these semi-supervised methods, we incorporate low-light consistency that facilitates learning explicit nighttime-robust representations without additional labeling.

==> include/table_fisheye_epe.tex <==
\begin{table}[h]
\centering

\caption{Endpoint-error results on datasets with diverse lens distortion.}
\label{tab:fisheye_epe}

\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\toprule
\textbf{Stage} & \textbf{SynWoodScape} & \textbf{Sintel - Clean} & \textbf{Sintel - Final} & \textbf{KITTI} \\ 
Sintel         & 5.12           & \textbf{1.94}    & \textbf{3.18}    & \textbf{5.10}  \\ 
Finetune       & \textbf{1.40}  & 5.44             & 10.32             & 14.34           \\ 
Joint          & 1.48           & 2.44             & 4.14             & 7.31           \\ 
\bottomrule
\end{tabular}
}

\vspace*{-3mm}

\end{table}

==> include/table_fisheye_schedule.tex <==
\begin{table}[h]

\vspace*{5mm}
\centering
\caption{Details of the training schedule. Column header abbreviations: LR: learning rate, BS: batch size, WD: weight decay, CS: crop size. Training dataset abbreviations: C: FlyingChairs, W: SynWoodScape, S: Sintel, T: FlyingThings3D, K: KITTI-2015, H: HD1K.}

\vspace*{5mm}

\begin{subtable}{\columnwidth}
\centering
\caption{Finetuning baseline. During the Sintel stage, the dataset distribution is S(.67), T(.12), K(.13), H(.08).}
% \vspace*{1mm}
\label{subtab:fisheye-ft}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\toprule
\textbf{Stage} & \textbf{Weights} & \textbf{Dataset} & \textbf{LR} & \textbf{BS} & \textbf{WD} & \textbf{CS}     \\ 
\midrule
Chairs   & -       & C             & 4e-4          & 6          & 1e-4         & {[}368, 496{]} \\ 
Things   & Chairs  & T             & 1.2e-4        & 3          & 1e-4         & {[}400, 720{]} \\ 
Sintel   & Things  & S+T+K+H       & 1.2e-4        & 3          & 1e-5         & {[}368, 768{]} \\ 
Finetune & Sintel  & W             & 1e-4          & 3          & 1e-5         & {[}600, 800{]} \\ 
\bottomrule
\end{tabular}
}
\end{subtable}

\vspace*{5mm}

\begin{subtable}{\columnwidth}
\centering
\caption{Jointly training baseline. During the Joint stage, the dataset distribution is W(.65), S(.17), T(.13), K(.03), H(.02).}
\vspace*{-2mm}
\label{subtab:fisheye-jt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|}
\toprule
\textbf{Stage} & \textbf{Weights} & \textbf{Dataset} & \textbf{LR} & \textbf{BS} & \textbf{WD} & \textbf{CS}     \\ 
\midrule
Chairs   & -       & C             & 4e-4          & 6          & 1e-4         & {[}368, 496{]} \\ 
Things   & Chairs  & T             & 1.2e-4        & 3          & 1e-4         & {[}400, 720{]} \\ 
Joint    & Things  & W+S+T+K+H     & 1e-4          & 3          & 1e-5         & {[}368, 768{]} \\ 
\bottomrule
\end{tabular}
}
\end{subtable}

\vspace*{1mm}

\end{table}
